Invertible Frowns: Video-to-Video Facial Emotion Translation

We present Wav2Lip-Emotion, a video-to-video translation architecture that modifies facial expressions of emotion in videos of speakers. Previous work modifies emotion in images, uses a single image to produce a video with animated emotion, or puppets facial expressions in videos with landmarks from a reference video. However, many use cases such as modifying an actor's performance in post-production, coaching individuals to be more animated speakers, or touching up emotion in a teleconference require a video-to-video translation approach. We explore a method to maintain speakers' lip movements, identity, and pose while translating their expressed emotion. Our approach extends an existing multi-modal lip synchronization architecture to modify the speaker's emotion using L1 reconstruction and pre-trained emotion objectives. We also propose a novel automated emotion evaluation approach and corroborate it with a user study. These find that we succeed in modifying emotion while maintaining lip synchronization. Visual quality is somewhat diminished, with a trade off between greater emotion modification and visual quality between model variants. Nevertheless, we demonstrate (1) that facial expressions of emotion can be modified with nothing other than L1 reconstruction and pre-trained emotion objectives and (2) that our automated emotion evaluation approach aligns with human judgements.

==> dataset_table.tex <==
\begin{table}
\begin{center}
\begin{tabular}{@{}lllll@{}}

\textbf{Dataset} & \textbf{Hours} & \textbf{Individuals} & \textbf{Emotion}  &\textbf{Intensity} \\ \toprule
\textit{Unreleased} &  &  &  &  \\
 MEAD full & 40 & 60 & 8 & 3 \\
 \midrule
 \textit{Released} &  &  &  &  \\
 MEAD train & $\sim$ 25 & 37 & 3 & 1 \\ 
 MEAD val & $\sim$ 3 & 5 & 3 & 1 \\ 
 MEAD test & $\sim$ 3 & 5 & 3 & 1 \\ 
 \bottomrule
 
 %CMU-MOSEI\cite{bagher-zadeh-etal-2018-multimodal} & 65 & 1000 & 6 & 4 \\ \bottomrule
 \end{tabular}
 \end{center}
\caption{The full MEAD data has not been completely released. On May 5th, 2021, a dataset of 47 actors was made available. We divide these 47 actors presently available into three splits, and only include happy, neutral, and sad emotions at one intensity due to pre-processing compute constraints.}
\label{tab:dataset}
\end{table}
